Learning Versatile Neural Architectures by Propagating Network Codes

This work explores how to design a single neural network capable of adapting to multiple heterogeneous vision tasks, such as image segmentation, 3D detection, and video recognition. This goal is challenging because both network architecture search (NAS) spaces and methods in different tasks are inconsistent. We solve this challenge from both sides. We first introduce a unified design space for multiple tasks and build a multitask NAS benchmark (NAS-Bench-MR) on many widely used datasets, including ImageNet, Cityscapes, KITTI, and HMDB51. We further propose Network Coding Propagation (NCP), which back-propagates gradients of neural predictors to directly update architecture codes along the desired gradient directions to solve various tasks. In this way, optimal architecture configurations can be found by NCP in our large search space in seconds. Unlike prior arts of NAS that typically focus on a single task, NCP has several unique benefits. (1) NCP transforms architecture optimization from data-driven to architecture-driven, enabling joint search an architecture among multitasks with different data distributions. (2) NCP learns from network codes but not original data, enabling it to update the architecture efficiently across datasets. (3) In addition to our NAS-Bench-MR, NCP performs well on other NAS benchmarks, such as NAS-Bench-201. (4) Thorough studies of NCP on inter-, cross-, and intra-tasks highlight the importance of cross-task neural architecture design, i.e., multitask neural architectures and architecture transferring between different tasks. Code is available at https://github.com/dingmyu/NCP.

==> supps/tables/cls_transfer.tex <==
\begin{table*}[t]
  \caption{Single-crop top-1 error rates (\%) of Network Propagation (NP) on the ImageNet validation set.
  The first three models are propagated using neural predictors that are trained on ImageNet-50-1000, ImageNet-50-100, ImageNet-10-1000, respectively.
  The last model is searched by joint optimization of all three predictors.
  $\lambda$ is set to 0.7 during the network propagation process for all searched models.
  FLOPs is measured using an input size of $224\times 224$. Part of this table has been shown in our main paper.
  }
  \centering
%   \footnotesize
  \scalebox{1}{
  \tabcolsep=0.33cm
  \begin{tabular}{l|rr|cc|cc|cc}
    \toprule        
    \multirow{2}{*}{Model} & \multirow{2}{*}{Params} & \multirow{2}{*}{FLOPs} & \multicolumn{2}{c|}{ImNet-50-1000} & \multicolumn{2}{c|}{ImNet-50-100} & \multicolumn{2}{c}{ImNet-10-1000} \\
    & & & top1 & top5 & top1 & top5 & top1 & top5\\
    \midrule
    ResNet$18$~\cite{he2016deep} & 11.20M & 1.82G & 82.72 & 93.88 & 53.04 & 77.64 & 85.00 & 97.40 \\
    ResNet$34$~\cite{he2016deep} & 21.31M & 3.68G & 83.40 & 94.28 & 52.52 & 77.20 & 87.00 & 98.00 \\
    ResNet$50$~\cite{he2016deep} & 23.61M & 4.12G & 83.76 & 94.48 & 50.16 & 75.12 & 86.00 & 98.00\\
    % ResNet$101$~\cite{he2016deep} & 42.60M & 7.85G & 84.32 & 94.80 & 51.92 & 75.72 & 86.00 & 97.80\\
    HRNet-W$18$s~\cite{wang2020deep} & 13.65M & 2.62G & 83.04 & 95.16 & 53.00 & 77.92 & 85.00 & 98.20 \\
    HRNet-W$18$~\cite{wang2020deep} & 19.35M & 4.33G & 83.48 & 94.04 & 50.28 & 76.60 & 83.80 & 98.80 \\
    HRNet-W$32$~\cite{wang2020deep} & 39.29M & 8.99G & 84.00 & 95.12 & 52.00 & 76.48 & 83.80 & 98.40 \\
    % HRNet-W$48$~\cite{wang2020deep} & 75.52M & 17.36G & 84.52 & 94.92 & 52.88 & 77.40 & 86.60 & 98.60 \\
    \midrule
    \textbf{\name-50-1000}~(Fig.~\ref{fig:dynamic-cls-07}) & 4.39M & 5.95G & \textbf{85.80} & 95.36 & 56.04 & 80.20 & 86.80 & 98.20\\
    \textbf{\name-50-100}~(Fig.~\ref{fig:dynamic-cls-50-100-07}) & 3.33M & 3.55G & 82.76 & 94.32 & 56.40 & 81.16 & 85.60 & 99.00\\
    \textbf{\name-10-1000}~(Fig.~\ref{fig:dynamic-cls-10-1000-07}) & 4.06M & 5.51G & 84.60 & 95.12 & 55.60 & 79.92 & 87.80 & \textbf{99.20} \\
    \textbf{\name-All}~(Fig.~\ref{fig:dynamic-cls-abc}) & 4.28M & 6.72G & 85.12 & \textbf{95.56} & \textbf{58.12} & \textbf{82.20} & \textbf{88.20} & 98.20 \\
    \bottomrule
  \end{tabular}
  }
  \label{tab:transfer_cls}
\end{table*}

==> supps/tables/seg_transfer_arxiv.tex <==
\begin{table*}[t]
    \caption{
    Comparative results (\%) of \alias~on the Cityscapes validation set. 
    The first two architectures are searched using neural predictors that are trained on the Cityscapes dataset with an input size of $512 \times 1024$ (Seg) and the resized Cityscapes dataset with an input size of $128 \times 256$ (Seg-4x), respectively. The last model is searched by joint optimization of both the two predictors. 
    $\lambda$ is set to 0.5 during the network codes propagation process. All models are trained from scratch. FLOPs is measured using $512\times 1024$.
    }
    \centering
    {
    % \footnotesize 
    \scalebox{1}{ 
    \tabcolsep=0.08cm
    \begin{tabular}{l|rr|ccc|ccc|ccc}
        \toprule
        \multirow{3}{*}{Method} & \multirow{3}{*}{Params} & \multirow{3}{*}{FLOPs} & \multicolumn{3}{c|}{Cityscapes} & \multicolumn{3}{c|}{Cityscapes} & \multicolumn{3}{c}{ADE20K} \\
        &&& \multicolumn{3}{c|}{$512 \times 1024$} & \multicolumn{3}{c|}{$128 \times 512$} & \multicolumn{3}{c}{$512 \times 512$} \\
        &&& mIoU & mACC & aACC & mIoU & mACC & aACC & mIoU & mACC & aACC \\
        \midrule
    ResNet$18$-PSP~\cite{zhao2017pyramid} & 12.94M & 108.53G & 73.21 & 79.86 & 95.51 & 62.66 & 70.17 & 93.25 & 33.45 & 40.95 & 77.78\\
    ResNet$34$-PSP~\cite{zhao2017pyramid} & 23.05M & 193.12G & 76.17 & 82.66 & 95.99 & 64.17 & 72.37 &  93.48 & 32.78 & 41.23 & 77.52\\
    % ResNet$50$-PSP~\cite{zhao2017pyramid} & 48.98M & 356.91G & 76.49 & 83.18 & 95.98 & 66.19 & 74.25 & 93.80 & 37.26 & 44.77 & 78.78\\
    HRNet-W$18$s~\cite{wang2020deep} & 5.48M & 22.45G & 76.21 & 84.43 & 95.86 & 64.49 & 73.58 & 93.71 & 34.39 & 44.65 & 77.60\\
    HRNet-W$18$~\cite{wang2020deep} & 9.64M & 37.01G & \textbf{77.73} & \textbf{85.61} & 96.20 & 65.19 & 74.85 & 93.66 & 34.84 & 45.27 & 77.80\\
	\midrule
	\textbf{\name-}$\mathbf{512 \times 1024}$~(Fig.~\ref{fig:dynamic-seg}) & 7.91M & 29.34G & 77.15 & 84.73 & 96.01 & 62.40 & 71.70 & 93.34 & 33.32 & 42.97 & 77.41 \\
	\textbf{\name-}$\mathbf{128 \times 512}$~(Fig.~\ref{fig:dynamic-4xseg}) & 2.61M & 31.37G & 70.91 & 80.20 & 95.21 & \textbf{65.89} & \textbf{75.19} & 93.79 & 27.52 & 35.88 & 73.85 \\
	\textbf{\name-Both}~(Fig.~\ref{fig:dynamic-segboth}) & 7.82M & 50.90G & 77.35 & 84.65 & \textbf{96.23} & 64.98 & 73.82 & \textbf{93.83} & \textbf{35.65} & \textbf{45.64} & \textbf{77.94} \\
    \bottomrule
    \end{tabular}
    }}
    \label{tab:transfer_seg}
\end{table*}

==> tables/3ddet.tex <==
\begin{table}[t]
    \caption{3D detection results based on the Pointpillar~\cite{lang2019pointpillars} framework on the KITTI split1 validation set. The 3D detection and bird's-eye view (BEV) detection AP (\%) on the car and pedestrian classes are reported.
    FLOPs is calculated for 2D RPN network using an input size of $496\times 432$.
    For ResNet~\cite{he2016deep}, the dilation rate of the convolution layers of the last two blocks are set to 2/4 to keep a 4 times larger stride, as in ~\cite{zhao2017pyramid}.
    Due to the limitation of GPU memories, ResNet$101$ and HRNet-W$48$ are not included.
    }
    \centering
    {
    \footnotesize 
    \scalebox{0.88}{ 
    \tabcolsep=0.1cm
    \begin{tabular}{l|rr|cc|cc}
        \toprule
        \multirow{1}{*}{Method} & Params & FLOPs & Car-3D & Car-BEV & Ped-3D & Ped-BEV \\
        % & [split1/split2/test] & [split1/split2/test] & [split1/split2/test] \
        \midrule
    ResNet$18$~\cite{he2016deep} & 13.25M & 55.47G & 75.49 & 87.57 & 43.34 & 49.68 \\
    ResNet$34$~\cite{he2016deep} & 23.80M & 97.77G & 76.97 & 87.75 & 46.32 & 52.50 \\
    ResNet$50$~\cite{he2016deep} & 53.34M & 178.50G & 76.80 & 87.16 & 44.71 & 51.56 \\
    HRNet-W$18$s~\cite{wang2020deep} & 8.24M & 17.70G & 76.40 & 87.59 & 41.83 & 46.45 \\
    HRNet-W$18$~\cite{wang2020deep} & 15.22M & 29.08G & 76.63 & 87.15 & 44.46 & 52.11 \\
    HRNet-W$32$~\cite{wang2020deep} & 35.21M & 71.03G & 77.71 & 88.74 & 47.41 & 53.20 \\
	Pointpillar~\cite{lang2019pointpillars} & 4.80M & 61.75G & 77.12 & 87.61 & 45.54 & 53.52\\
	\midrule
	\textbf{\name-Car} & 2.73M & 33.25G &  \textbf{78.13} & \textbf{88.95} & 45.51 & 53.26 \\
	\textbf{\name-Ped} & 2.99M & 44.46G &  77.98 & 87.96 & \textbf{48.71} & \textbf{54.34} \\
    \bottomrule
    \end{tabular}
    }}
    \label{tab:overall_3ddet}
    \vspace{-6pt}
\end{table}

==> tables/ablation.tex <==
\begin{table}
  \caption{Comparison of different traversal methods on the Cityscapes validation set. `wta' -- winner-takes-all. }
  \centering
  \footnotesize
  \scalebox{1}{
  \tabcolsep=0.12cm
  \begin{tabular}{lrrccc}
    \toprule        
    Model & Params & FLOPs & mIoU & mAcc & aAcc \\
    \midrule
    Random search + top-K & 6.74M & 44.32G & 77.66 & 85.35 & 96.13  \\
    NetAdapt~\cite{yang2018netadapt} & 10.83M & 42.49G & 78.02 & 85.68 & 96.24 \\
    NP-continuous & 8.39M & 36.25G & \textbf{78.36} & \textbf{86.24} & \textbf{96.29} \\
    NP-winner takes all & 7.18M & 32.88G & 77.91 & 85.69 & 96.23 \\
    \bottomrule
  \end{tabular}
  }
  \label{tab:ablation}
  \vspace{-8pt}
\end{table}


==> tables/baseline_cls.tex <==
\begin{figure}[t]
\begin{minipage}[t]{0.46\linewidth}
\begin{table}[H]
  \caption{Comparative results (\%) on the Cityscapes validation set. All models are trained from scratch. FLOPs is measured using an input size of $512\times 1024$. $\lambda=0.7,~0.3,~0.1$ for `S', `M', and `L'. The hyperparameter optimization methods Random Search~\cite{li2020random}, NetAdapt~\citep{yang2018netadapt}, and Neural Predictor~\citep{wen2020neural}
  }
  \centering
  \footnotesize
  \resizebox{1\linewidth}{!}{%
  \tabcolsep=0.07cm
  \begin{tabular}{l|rr|ccc}
    \toprule        
    Model & Params & FLOPs & mIoU & mAcc & aAcc \\
    \midrule
    Random Search & 16.27M & 130.50G & 77.66 & 85.35 & 96.13 \\
    NetAdapt & 10.83M & 42.49G & 78.02 & 85.68 & 96.24 \\
    Neural Predictor & 33.49M & 182.60G & 78.89 & 86.46 & 96.21 \\
    % \midrule
    % Auto-DeepLab & 10.15M & 289.78G & 79.74 & $-$ & $-$ \\
    % Darts~\citep{hanxiao2019darts} & 10.15M & 289.78G & 79.74 & $-$ & $-$ \\
    \midrule
    ResNet$18$-PSP & 12.94M & 108.53G & 73.21 & 79.86 & 95.51  \\
    ResNet$34$-PSP & 23.05M & 193.12G & 76.17 & 82.66 & 95.99 \\
    HRNet-W$18$ & 9.64M & 37.01G & 77.73 & 85.61 & 96.20 \\
    \midrule
    \textbf{\name-M-wta} & 7.18M & 32.88G & 77.91 & 85.69 & 96.23 \\
    \textbf{\name-S} & 6.04M & 20.07G & 76.98 & 85.14 & 96.07 \\
    \textbf{\name-M} & 8.39M & 36.25G & 78.36 & 86.24 & 96.29 \\
    \textbf{\name-L} & 37.70M & 179.98G & \textbf{80.05} & \textbf{87.12} & \textbf{96.49} \\
    \bottomrule
  \end{tabular}
  }
  \label{tab:baseline}
  \vspace{-6pt}
\end{table}
\end{minipage}
\hfill
\begin{minipage}[t]{0.50\linewidth}
\begin{table}[H]
  \caption{Top-1 error (\%) on the ImageNet validation set.
  `Cls-A', `Cls-B', `Cls-C' denote the predictor is trained on benchmarks of ImageNet-50-1000, ImageNet-50-100, ImageNet-10-1000, respectively. `Cls-ABC' searches a multitask architecture using all three predictors.
  FLOPs is measured using input size $224\times 224$. $\lambda=0.7$. Top-2 results are highlighted in \textbf{bold}.
  }
  \centering
  \footnotesize
  \resizebox{1\linewidth}{!}{%
  \tabcolsep=0.15cm
  \begin{tabular}{l|rr|ccc}
    \toprule        
    Model & Params & FLOPs & Cls-A & Cls-B & Cls-C \\
    \midrule
    ResNet$50$ & 23.61M & 4.12G & 83.76 & 50.16 & 86.00 \\%& 76.6 \\
    ResNet$101$ & 42.60M & 7.85G & 84.32 & 51.92 & 86.00 \\%& 78.2 \\
    HRNet-W$32$ & 39.29M & 8.99G & 84.00 & 52.00 & 83.80 \\%& 78.5 \\
    HRNet-W$48$ & 75.52M & 17.36G & 84.52 & 52.88 & 86.60\\%& 79.3\\
    % \midrule
    % Neural Predictor-A~\cite{wen2020neural}& 12.95M & 15.36G & 85.04 & 50.60 & 85.00 \\
    % Neural Predictor-B~\cite{wen2020neural}& 10.22M & 15.77G & 82.04 & 52.60 & 85.80 \\
    % Neural Predictor-C~\cite{wen2020neural}& 27.97M & 26.64G & 84.56 & 50.48 & 87.60 \\
    \midrule
    \textbf{\name-A} & 4.39M & 5.95G & \st{85.80} & 56.04 & 86.80 \\
    \textbf{\name-B} & 3.33M & 3.55G & 82.76 & \nd{56.40} & 85.60 \\
    \textbf{\name-C} & 4.06M & 5.51G & 84.60 & 55.60 & \nd{87.80} \\
    \midrule
    \textbf{\name-ABC} & 4.28M & 6.72G & \nd{85.12} & \st{58.12}  & \st{88.20}  \\
    \bottomrule
  \end{tabular}
  }
  \label{tab:overall_cls}
  \vspace{-4pt}
\end{table}
\end{minipage}
\vspace{-8pt}
\end{figure}




==> tables/seg.tex <==
\begin{table}
  \caption{Comparative results (\%) on the Cityscapes validation set. All models are trained from scratch. FLOPs is measured using an input size of $512\times 1024$. $\lambda=0.7,~0.3,~0.1$ for `S', `M', and `L'.
  }
  \centering
  \footnotesize
  \scalebox{0.8}{
  \tabcolsep=0.12cm
  \begin{tabular}{l|rr|ccc}
    \toprule        
    Model & Params & FLOPs & mIoU & mAcc & aAcc \\
    \midrule
    ResNet$18$-PSP~\citep{zhao2017pyramid} & 12.94M & 108.53G & 73.21 & 79.86 & 95.51  \\
    ResNet$34$-PSP~\citep{zhao2017pyramid} & 23.05M & 193.12G & 76.17 & 82.66 & 95.99 \\
    ResNet$50$-PSP~\citep{zhao2017pyramid} & 48.98M & 356.91G & 76.49 & 83.18 & 95.98 \\
    ResNet$101$-PSP~\citep{zhao2017pyramid} & 67.97M & 512.28G & 78.41 & 85.17 & 96.29\\
    HRNet-W$18$s~\citep{wang2020deep} & 5.48M & 22.45G & 76.21 & 84.43 & 95.86\\
    HRNet-W$18$~\citep{wang2020deep} & 9.64M & 37.01G & 77.73 & 85.61 & 96.20 \\
    HRNet-W$32$~\citep{wang2020deep} & 29.55M & 90.55G & 79.28 & 86.48 & 96.31 \\
    HRNet-W$48$~\citep{wang2020deep} & 65.86M & 187.21G & 79.37 & 86.72 & 96.36 \\
    \midrule
    NetAdapt~\citep{yang2018netadapt} & 10.83M & 42.49G & 78.02 & 85.68 & 96.24 \\
    Random Search~\citep{li2020random} & 16.27M & 130.50G & 77.66 & 85.35 & 96.13 \\
    Neural Predictor~\citep{wen2020neural} & 33.49M & 182.60G & 78.89 & 86.46 & 96.21 \\
    Auto-DeepLab~\citep{liu2019auto} & 10.15M & 289.78G & 79.74 & $-$ & $-$ \\
    \midrule
    \textbf{\name-M-winner takes all} & 7.18M & 32.88G & 77.91 & 85.69 & 96.23 \\
    \textbf{\name-S-continuous} & 6.04M & 20.07G & 76.98 & 85.14 & 96.07 \\
    \textbf{\name-M-continuous} & 8.39M & 36.25G & 78.36 & 86.24 & 96.29 \\
    \textbf{\name-L-continuous} & 37.70M & 179.98G & \textbf{80.05} & \textbf{87.12} & \textbf{96.49} \\
    \bottomrule
  \end{tabular}
  }
  \label{tab:overall_seg}
  \vspace{-6pt}
\end{table}


==> tables/video.tex <==
\begin{table}[t]
    \caption{Video recognition results on the HMDB51 dataset. FLOPs is calculated using an input size of $112\times 112$.
    The last 2D convolutional layer before the final classifier is replaced with a 3D convolutional layer ($3 \times 3 \times 3$) for all models.
    Video transfer.
    }
    \centering
    {
    \footnotesize 
    \scalebox{0.96}{ 
    \tabcolsep=0.15cm
    \begin{tabular}{l|rr|cc|cc}
        \toprule
        \multirow{2}{*}{Method} & \multirow{2}{*}{Params} & \multirow{2}{*}{FLOPs} & \multicolumn{2}{c}{Scratch} & \multicolumn{2}{c}{Pretrained} \\
        &&& top1 & top5 & top1 & top5 \\
        \midrule
    ResNet$18$~\cite{he2016deep} & 12.10M & 0.59G & 21.53 & 55.69 & 27.84 & 60.50 \\
    ResNet$34$~\cite{he2016deep} & 22.21M & 1.20G & 19.89 & 52.94 & 31.22 & 63.53\\
    ResNet$50$~\cite{he2016deep} & 25.41M & 1.35G & 15.48 & 49.19 & 32.11 & 62.72 \\
    ResNet$101$~\cite{he2016deep} & 44.39M & 2.56G & 15.17 & 47.72 & 28.55 & 65.11\\
    HRNet-W$18$s~\cite{wang2020deep} & 14.35M & 0.86G & 24.55 & 55.87 & 30.96 & 61.21 \\
    HRNet-W$18$~\cite{wang2020deep} & 20.05M & 1.41G & 24.11 & 55.33 & 32.48 & 64.30\\
    HRNet-W$32$~\cite{wang2020deep} & 40.67M & 2.93G & 23.22 & 56.13 & \textbf{34.16} & \textbf{66.45} \\
    HRNet-W$48$~\cite{wang2020deep} & 77.09M & 5.67G & 18.75 & 40.62 & 30.51 & 65.13\\
	\midrule
	\textbf{\name-S} & 3.87M & 0.73G & 26.95 & 60.76 & 32.74 & 63.07\\
	\textbf{\name-M} & 4.71M & 1.00G & \textbf{28.73} & \textbf{61.83} & 32.82 & 62.28\\
	\textbf{\name-L} & 6.05M & 1.51G & 26.51 & 58.63 & 33.01 & 65.04\\
    \bottomrule
    \end{tabular}
    }}
    \label{tab:overall_video}
    \vspace{-6pt}
\end{table}
